Autoresearch for Marketplace Catalogs: From Legacy Forms to AI-Native Matching

Two-sided service marketplaces are moving from deterministic request-form intake to AI-native probabilistic matching, enabled by large language models (LLMs) that infer intent, preferences, and latent constraints from natural language. Relying on inferred intent rather than fixed-form fields forces these platforms to regenerate the provider-side preference taxonomy underwriting matching, search, and pricing: attributes interpretable to service providers while remaining a useful signal for marketplace decisions. We present an autoresearch loop that generates this taxonomy, one occupation at a time, and has been deployed in production at a major U.S. consumer services marketplace since April 2026, spanning 132 occupations. Instead of one global hierarchy, the loop treats each occupation as an independent generation problem and runs iterative propose-evaluate-keep refinement cycles. Each candidate tag set is scored by a recalibrated six-rubric LLM-as-judge framework, and a 7-critic panel of distinct personas contributes weighted penalties to an adjusted score, with no hard vetoes. A separate parity-mapping stage maps legacy request-form Q&A pairs back to the generated taxonomy, yielding both a coverage signal and an interface for human quality assurance; it does so by first inferring the provider attribute each legacy question was meant to measure, rather than translating questions to tags literally.

==> tex-figures/stepback_abstraction.tex <==
% S2 publication diagram 2 — Underlying-attribute abstraction for legacy migration
% Style: B&W with bold accent on the abstraction step (the data-normalization layer).
% Loaded via \input{figures/stepback_abstraction.tex} inside a figure env.
\begin{tikzpicture}[
    >={Stealth[length=2.2mm]},
    node distance=8mm and 14mm,
    every node/.style={font=\small},
    box/.style={draw, very thin, rectangle, rounded corners=1pt,
                fill=black!4, minimum height=8mm, minimum width=30mm,
                align=center, inner sep=3pt},
    boxAccent/.style={draw, semithick, rectangle, rounded corners=1pt,
                     fill=black!12, minimum height=8mm, minimum width=30mm,
                     align=center, inner sep=3pt},
    data/.style={draw, very thin, rectangle, fill=white,
                 minimum height=7mm, minimum width=28mm,
                 align=center, inner sep=3pt},
    annot/.style={font=\footnotesize\itshape, align=center},
]
  % --- Naive path (top, shown crossed out as the alternative we reject)
  \node[data]                          (qa)         {Legacy Q\&A pair\\(per category)};
  \node[box, right=of qa]              (literal)    {Literal translation\\``answer $\to$ sub-tag''};
  \node[data, right=of literal]        (union)      {Unioned legacy\\schema (bad)};

  \draw[->] (qa) -- (literal);
  \draw[->] (literal) -- (union);

  \node[annot, above=1mm of literal.north] {(a) naive translation};

  % cross through the union output
  \draw[very thick, gray] (union.north west) -- (union.south east);
  \draw[very thick, gray] (union.north east) -- (union.south west);

  % --- Our path (bottom)
  \node[data, below=14mm of qa]        (qa2)        {Legacy Q\&A pair\\(per category)};
  \node[boxAccent, right=of qa2]       (abstract)   {Abstraction prompt:\\``what underlying\\attribute is this?''};
  \node[data, right=of abstract]       (attr)       {Underlying job\\attribute (e.g.\\\emph{Pipe material})};
  \node[box, right=of attr]            (gen)        {Catalog\\generator};

  \draw[->] (qa2) -- (abstract);
  \draw[->] (abstract) -- (attr);
  \draw[->] (attr) -- (gen);

  \node[annot, above=1mm of abstract.north] {(b) underlying-attribute abstraction};

  % --- Parity check (side branch)
  \node[box, below=10mm of attr] (parity) {Parity check\\(legacy $\to$ new tag)};
  \draw[->, dashed] (qa2.south) |- ([yshift=2mm]parity.west);
  \draw[->, dashed] (gen.south) |- ([yshift=2mm]parity.east);
  \node[annot, below=1mm of parity.south] {coverage signal $\to$ Parity critic};

\end{tikzpicture}

